Unsupervised Relation Extraction from Language Models using Constrained Cloze Completion

We show that state-of-the-art self-supervised language models can be readily used to extract relations from a corpus without the need to train a fine-tuned extractive head. We introduce RE-Flex, a simple framework that performs constrained cloze completion over pretrained language models to perform unsupervised relation extraction. RE-Flex uses contextual matching to ensure that language model predictions matches supporting evidence from the input corpus that is relevant to a target relation. We perform an extensive experimental study over multiple relation extraction benchmarks and demonstrate that RE-Flex outperforms competing unsupervised relation extraction methods based on pretrained language models by up to 27.8 $F_1$ points compared to the next-best method. Our results show that constrained inference queries against a language model can enable accurate unsupervised relation extraction.

==> experiments_old.tex <==
\section{Experimental Evaluation}\label{sec:experiments}
We evaluate the performance of \system. The main points we seek to validate are: (1) how accurately can \system extract relations by utilizing contextual evidence, (2) what are the limitations of \system, and (3) what is the impact of different components of \system on the quality of the extracted repairs. We evaluate \system against several competing relation extraction methods on four relation extraction benchmarks. We also perform a detailed error analysis to understand when \system is more effective than methods that rely on fine-tuning. Finally, we perform several micro-benchmark experiments to analyze each component of \system. 

% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{l|l|l|l|l|l}
% \textbf{Benchmark} & \textbf{Relation in Context} & \textbf{Extraction Type} & \textbf{Underlying Corpus} & \textbf{\# of Relations} & \textbf{Total Samples}\\\hline T-REx & \makecell[l]{Implicit Relation \\ Mention} & Single-Token & Wikipedia & 41 & 34,039\\\hline
% Google-RE & \makecell[l]{Exact Relation \\ Mention} & Single-Token & Wikipedia & 3 & 5,528\\\hline
% ZSRE & \makecell[l]{Possibly Irrelevant \\ Context} & \makecell[l]{Multi-Token} & Wikipedia & 120 & 42,635\\\hline
% TACRED & \makecell[l]{Possibly Irrelevant \\ Context} & \makecell[l]{Multi-Token} & TAC-KBP & 41 & 6,357\\
% \end{tabular}
% \caption{We consider four benchmarks that vary with respect to the type of target extractions, the quality of context to relation alignment, and the underlying corpus.}
% \label{tab:benchmarks}
% \end{table*}

\subsection{Experimental Setup}\label{sec:exp_setup}
We describe the benchmarks, metrics, and methods we use in our evaluation. We discuss implementation details in the Appendix.

\subsubsection{Datasets and Benchmarks}\label{sec:datasets}

We consider four benchmarks that vary in three characteristics: (1) whether extractions correspond to multi-token or single-token spans, (2) the degree to which the context associated with each query expresses evidence of the relation, and (3) the underlying corpus the examples were chosen from. The central reason for for varying the characteristics of the datasets are that the existing methods for general relation extraction tend to be limited with respect to one of the varying aspects, so we wish to consider at least one setting the method was specifically designed for. A number of existing benchmarks, for instance, assume that the answer to the query exists in the associated context. We include datasets which fairly can compare to these benchmarks. A summary of the dataset characteristics is shown in Table~\ref{tab:benchmarks}. The three datasets that use Wikipedia as the underlying corpus draw their relations from Wikidata \cite{vrandevcic2012wikidata}, while the TACRED dataset \cite{zhang2017tacred} uses relations from the TAC Knowledge Base Population challenge \cite{mcnamee2009overview}.

\newparagraph{T-REx} We consider 41 relations from the T-REx dataset~\cite{elsahar_t-rex:_nodate}, which algorithmically aligns each fact tuple to a set of contexts in Wikipedia. This dataset was used previously to show that language models can act as primitive knowledge bases \cite{petroni-etal-2019-language}. We consider the same dataset, with a single token restriction on the expected responses, and require an extraction from each example.

\newparagraph{Google-RE} We consider 3 single-token relations in the Google-RE dataset. We consider samples for which human annotators have manually verified the target relation is expressed. Like T-REx, this dataset was previously used in \citet{petroni-etal-2019-language}.

\newparagraph{Zero-Shot Relation Extraction (ZSRE)} The Zero Shot Relation Extraction Benchmark was created by \citet{levy_zero-shot_2017} to test how well relation extraction systems can generalize to unseen relations. The dataset contains 120 relations. We consider the test set of this benchmark, filtered to exclude repeated instances. This dataset contains contexts with no evidence of the relation, and thus, for these examples the correct behavior is to return no answer.

\newparagraph{TAC Relation Extraction Dataset (TACRED)} The TAC Relation Extraction Dataset \cite{zhang2017position} is a relation classification dataset. The original task is to predict the relation of a subject and object pair given a supporting context. There are 41 possible relations, with an additional relation labelled ``no\_relation" to denote an example whose sentence does not express the relation between the subject and object. We convert the dataset to our slot filling setting by considering the subject and relation known for each example, and setting the task to predict the object. Following the established process of \citet{levy_zero-shot_2017} for adding realistic negative examples, we distribute all examples labelled \texttt{no\_relation} to relations sharing the same head entity, and set the target object for each to be $\varnothing$.



% \newparagraph{Google-RE} We consider the setup provided in the LAMA probe by \citet{petroni-etal-2019-language}. We consider three relations from the Google-RE benchmark. We only consider samples for which human annotators have manually verified the target relation is expressed. We define a cloze template and a question for each relation.

% \newparagraph{T-REx} We consider 41 relations from the T-REx dataset~\cite{elsahar_t-rex:_nodate}, which algorithmically aligns each fact tuple to a set of contexts in Wikipedia. Unlike Google-RE, contexts may not have explicit evidence of the relation. We again consider the same samples provided by the LAMA probe~\cite{petroni-etal-2019-language}. We define a cloze template and a question for each relation.

% \begin{table}
% \centering
% \small
% \begin{tabular}{l|l} 
% \textbf{Property} & \textbf{Value} \\\hline
% Total samples & 42,635 \\
% \# of relations  & 120 \\
% \# of no answer samples & 17,878 \\
% \# of single token samples & 10,387 \\
% \# of multi-token samples & 14,370 \\
% Mean token length & 1.96 \\
% \end{tabular}
% \caption{Dataset statistics for the Zero-Shot Relation Extraction benchmark.}
% \label{tab:zsre_stats}
% \end{table}

% \newparagraph{Zero-Shot Relation Extraction (ZSRE)} The Zero Shot Relation Extraction Benchmark was created by \citet{levy_zero-shot_2017} to test how well relation extraction systems can generalize to unseen relations. The dataset contains 120 relations, with 10 folds of train/dev/test splits. We concatenate all test splits, filter any repeated examples, and consider the result to be our benchmark. Additionally, we sample up to 50 examples for each relation from the train and dev sets (ensuring no overlap with test instances) to produce our own dev split in order to tune hyperparameters. A summary of the dataset characteristics is provided in Table~\ref{tab:zsre_stats}. This benchmark is the most challenging: contexts that contain no evidence of the relation must be rejected, and the expected answer is a variable length span.

% \begin{table*}[t]
% \centering
% \begin{tabular}{l l|c|c c c c | c c c}
% \multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{Unsupervised}& \multicolumn{1}{l|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{} \\ 
% \cline{3-10}& & RE-Flex & NC & GD & UE-QA & SE-QA & BiDAF & B-Squad & B-ZSRE \\ \hline
% \multirow{2}{*}{T-REx} & \textbf{EM} & \textbf{56.0} & \red{22.9} & \red{43.2} & \red{14.2} & \red{21.2} & \red{35.5} & \red{42.2} & \red{46.2}\\
% & \textbf{F1} & \textbf{56.0} & \red{22.9} & \red{43.7} & \red{19.3} & \red{28.2} & \red{46.6} & \red{52.0} & \red{52.7}\\ \hline
% \multirow{2}{*}{Google-RE} & \textbf{EM} & \textbf{87.2} & \red{5.6} & \red{75.6} & \red{51.9} & \red{19.7} & \red{53.9} & \red{52.9} & \red{70.5}\\
% & \textbf{F1} & \textbf{87.2} & \red{5.6} & \red{75.7} & \red{65.0} & \red{25.3} & \red{74.8} & \red{76.5} & \red{75.8}\\ \hline
% \multirow{2}{*}{ZSRE} & \textbf{EM} & 43.7 & \red{14.1} & \red{9.3} & \red{16.7} & \red{17.3} & \red{40.2} & \blue{66.5} & \blue{\textbf{82.0}}\\
% & \textbf{F1} & 46.9 & \red{14.9} & \red{12.3} & \red{23.7} & \red{24.9} & \blue{49.0} & \blue{74.1} & \blue{\textbf{84.8}}\\ \hline
% \multirow{2}{*}{TACRED} & \textbf{EM} & 49.4 & \red{9.0} & \red{7.2} & \red{17.5} & \red{13.9} & \red{49.3} & \blue{\textbf{56.9}} & \blue{54.4}\\
% & \textbf{F1} & 50.1 & \red{9.0} & \red{7.9} & \red{22.0} & \red{18.6} & \blue{53.7} & \blue{\textbf{61.1}} & \blue{55.3}\\

% \hline
% \end{tabular}
% \caption{Performance for all methods on the four benchmarks. Bold values highlight the best method. \red{Red} and \blue{blue} values denote worse or better performance than RE-Flex, respectively.}
% \label{tab:overall_results}
% \end{table*}

\subsubsection{Competing Methods}\label{sec:methods}

We consider competing methods that support general relation extraction. We first consider two baselines that only use the language model, similar to our method: 

\newparagraph{Naive Cloze (NC)} We use the approach of \citet{petroni-etal-2019-language} which issues cloze queries without a context against the language model.

\newparagraph{Greedy Decoding with Context Seed (GD)} We consider greedily decoding an answer to a query, previously used to show that language models can primitively perform many natural language tasks \cite{radford2019language}. We prepend the relational cloze query with a context, and greedily decode an answer until an end of sequence or period token is emitted.

\newparagraph{}We also consider a number of extractive QA models:

\newparagraph{Unsupervised Extractive QA (UE-QA)} This method was proposed by~\citet{lewis_unsupervised_2019} and uses a self-supervised method to train a QA head over BERT-large. To form QA pairs, sentences are sampled from the input corpus, the sentences are masked to form cloze statements, and finally an unsupervised Neural Machine Translation model translates the cloze statement to a question. We replicate the method by training a BERT-Large-based QA model \cite{wolf2019transformers} using the author-provided data. The model is designed for the Squad1.0 QA setting, where the context is assumed to contain the answer to the query, and thus, it cannot reject irrelevant contexts to a query.

\newparagraph{Semi-supervised Extractive QA (SE-QA)} This method was proposed by~\citet{dhingra_simple_2018} as a semi-supervised approach to QA. It uses an off-the-shelf NER system to generate cloze-based question-answer pairs. The QA model is then trained directly on the generated cloze statements. \citet{dhingra_simple_2018} also provide their training data, which we use to train a BERT-Large-based QA model. This model also cannot reject irrelevant contexts.

\newparagraph{BiDAF trained on Squad 2.0 (BiDAF)} We train BiDAF \cite{seo2016bidirectional}, extended to be able to predict no answer \cite{levy_zero-shot_2017}, on Squad 2.0~\cite{rajpurkar-etal-2018-know}. BiDAF is a popular reading comprehension model that has previously been demonstrated to be effective for relation extraction. For Google-RE and T-REx, where an answer always exists, we ignore no-answer predictions and choose the next-best answer to be the output extraction.

\newparagraph{BERT-Large fine-tuned on Squad 2.0 (B-Squad)} We train BERT-Large on Squad 2.0. BERT-Large fine-tuned on Squad 2.0 performs similarly to state of the art question answering models. We follow the same protocol as above to always emit an answer if the dataset requires it.

\newparagraph{BERT-Large fine-tuned on ZSRE (B-ZSRE)} We train BERT-Large on the first train fold of the ZSRE benchmark. It's possible that the trained model has seen examples from the ZSRE test benchmark at train time because the benchmark is a concatenation of all test folds. This likely inflates this model's performance on the ZSRE dataset. However, we still include the model as a supervised QA model trained on relation extraction data.  We follow the same protocol as above to always emit an answer if the dataset requires it.

% We consider competing methods that support general relation extraction. We first consider a {\em baseline} that only use the language model: 
% \newparagraph{Naive Cloze (NC)} We use the approach of \citet{petroni-etal-2019-language} which issues cloze queries without a context against the language model. 

% We also consider approaches that combine language models with extractive QA models:

% \newparagraph{Unsupervised Extractive QA (UE-QA)} This method was proposed by~\citet{lewis_unsupervised_2019} and uses a self-supervised method to train a QA head over BERT-large. To form QA pairs, sentences are sampled from the input corpus, the sentences are masked to form cloze statements, and finally an unsupervised Neural Machine Translation model translates the cloze statement to a question. We replicate the method by training a BERT-Large-based QA model \cite{wolf2019transformers} using the author-provided data. The model is designed for the Squad1.0 QA setting, where the context is assumed to contain the answer to the query, and thus, it cannot reject irrelevant contexts to a query.

% \newparagraph{Semi-supervised Extractive QA (SE-QA)} This method was proposed by~\citet{dhingra_simple_2018} as a semi-supervised approach to QA. It uses an off-the-shelf NER system to generate cloze-based question-answer pairs. The QA model is then trained directly on the generated cloze statements. \citet{dhingra_simple_2018} also provide their training data, which we use to train a BERT-Large-based QA model. This model also cannot reject irrelevant contexts.

% \newparagraph{BERT-Large fine-tuned on Squad 2.0 (B-Squad)} We train BERT-Large on Squad 2.0~\cite{rajpurkar-etal-2018-know}. For Google-RE and T-REx, where an answer always exists, we ignore no-answer predictions and choose the next-best answer to be the output extraction.

% \newparagraph{BERT-Large fine-tuned on ZSRE (B-ZSRE)} This approach is similar to the previous one but here we train a BERT-Large-based QA model on the ZSRE train dataset. 

% \noindent The last two approaches are equivalent to that of \citet{levy_zero-shot_2017} on zero-shot relation extraction.

% \subsubsection{Evaluation Setup}\label{sec:eval_setup}

% \newparagraph{Evaluation Metrics} Following standard metrics from Squad 1.0~\cite{rajpurkar-etal-2016-squad}, we evaluate the quality of each extraction using two metrics: {\em Exact Match (EM)} and $F_1$-score. Exact match assigns a score of $1.0$ to a relation extraction when the extracted span matches exactly the ground truth span, otherwise it assigns a score of $0.0$. $F_1$ treats the extracted span as a set and considers the precision and recall (at the token level) between tokens in the predicted span and tokens in the ground truth span. For each relation, we compute the average EM and $F_1$ scores and then average these scores across relations. In the last step, we do not assign different weights to different relations. This approach enables us to understand the performance of the model across different relations better.

%\newparagraph{Implementation Details} Unless otherwise stated, we set \system's $\lambda$ parameter (see Section~\ref{sec:context_rejection}) to $0.0$ and the top-$k$ parameter (see Section~\ref{sec:alignment}) to $10$. We use Fairseq's implementation of RoBERTa-large\footnote{\url{https://github.com/pytorch/fairseq}} as our pretrained language model, and use the LAMA probe experiment setup~\footnote{\url{https://github.com/facebookresearch/LAMA}} as a starting point for our own experiments. For the embeddings of the context rejection mechanism, we use the FastText library. For the token embeddings of the alignment model, we first collect an embedding for each subword (RoBERTa uses byte-pair subword encodings) by concatenating the output representation of all 12 of the RoBERTa-large decoder layers for each subword. Because we operate on the token and not the subword level, we obtain a token representation by averaging all subword vector embeddings that compose a token. Examining the effect of our embedding choices is out of the scope of this work, and we leave it as a future analysis. For named entity recognition and noun phrase chunking (used for identifying multi-token extractions in \system), we use the default models of the Spacy library. We train and run all models on a single NVIDIA V100 32GB memory GPU.

% \begin{table*}[t]
% \centering
% \begin{tabular}{l|l l |l l |l l|l l}
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{T-REx}} & \multicolumn{2}{c|}{\textbf{Google-RE}} & \multicolumn{2}{c|}{\textbf{ZSRE}} & \multicolumn{2}{c}{\textbf{TACRED}} \\ \cline{2-9}
% & \textbf{EM} & \textbf{$\mathbf{F_1}$} & \textbf{EM} & \textbf{$\mathbf{F_1}$} & \textbf{EM} & \textbf{$\mathbf{F_1}$} & \textbf{EM} & \textbf{$\mathbf{F_1}$} \\ \hline
% NC      & 22.9 & 22.9 & 5.6  & 5.6  & 14.1 & 14.9 & 9.0  & 9.0 \\
% GD      & 43.2 & 43.7 & 75.6 & 75.7 & 9.3  & 12.3 & 7.2  & 7.9 \\ \hline
% UE-QA   & 14.2 & 19.3 & 51.9 & 65.0 & 16.7 & 23.7 & 17.5 & 22.0 \\
% SE-QA   & 21.2 & 28.2 & 19.7 & 25.3 & 17.3 & 24.9 & 13.9 & 18.6 \\ \hline
% BiDAF   & 35.5 & 46.6 & 53.9 & 74.8 & 40.2 & 49.0 & 49.3 & 53.7 \\
% B-Squad    & 42.2 & 52.0 & 52.9 & 76.5 & 66.5 & 74.1 & \textbf{56.9} & \textbf{61.1} \\
% B-ZSRE    & 46.2 & 52.7 & 70.5 & 75.8 & \textbf{82.0} & \textbf{84.8} & 54.4 & 55.3 \\ \hline
% \system & \textbf{56.0} & \textbf{56.0} & \textbf{87.2} & \textbf{87.2} & 43.7 & 46.9 & 49.4 & 50.1 \\
% \hline
% \end{tabular}
% \caption{Performance for all methods on the four benchmarks. Bold values highlight the best method.}
% \end{table*}



\subsection{Overall performance}\label{sec:overall}
We present the overall performance of all methods on all four benchmarks. The results are outlined in Table~\ref{tab:overall_results}. As shown, \system outperforms all unsupervised QA-based methods for all benchmarks yielding performance improvements of up to 27.8 $F_1$ points compared to the next-best method. Moreover, in two out of the four benchmarks (i.e., T-REx and Google-RE) \system  even yields improvements of 3.3 and 11.4 $F_1$ points compared to the best performing \emph{supervised} method.

\newparagraph{Comparison to Unsupervised Methods} RE-Flex consistently outperforms all unsupervised methods. In the basic settings of T-REx and Google-RE, where the answer always exists in the provided context, RE-Flex's smoothing approach outperforms both the naive generative ability of language models and the unsupervised question answering heads. These results highlight how RE-Flex mitigates the limitations of both groups of models. RE-Flex is able to apply the same constraints a question answering head imposes (the answer is a contiguous span in the provided context), without suffering from noisily aligned training data.

In the more realistics settings of ZSRE and TACRED, where contexts must be determined to express the relation, we again see a large gap between RE-Flex's performance and that of unsupervised models. Here, we additionally see the benefits of our proposed approach to filter contexts which do not contain evidence that the relation is expressed. In Section \ref{sec:context_rejection}, we futher explore how much adding the context filtering step benefits our approach.

\newparagraph{Comparison to Supervised Methods} We see the surprising result that RE-Flex outperforms even supervised baselines in the T-REx and Google-RE settings. This result shows that reasoning about contextual embeddings directly instead of training classifiers on top of them is a promising direction for relation extraction. In Section \ref{sec:perf_analysis}, we break down the errors of the QA models for these datasets to further analyze this result.

In the ZSRE and TACRED benchmarks, supervised QA methods generally outperform RE-Flex, with the exception of the BiDAF model, which exhibits similar performance. This result is to be expected, as the models benefit from annotated information about answer containment and explicit associations between entities in the query and the provided context.

% \begin{figure}
% \center
% \includegraphics[width=0.48\textwidth]{figures/deltaf1.pdf}
% \caption{Histogram breakdown of differences between $F_1$ performances between \system and supervised methods.}
% %\includegraphics[width=8cm]{Plot}
% \centering
% \label{fig:deltaf1}
% \end{figure}

Still, for many individual relations RE-Flex can perform competitively. We compute the difference in $F_1$ scores between 
\system and each of B-Squad and B-ZSRE for each relation in the ZSRE dataset, which contains the most diverse set of relations. The histograms of these differences can be found in Figure \ref{fig:deltaf1}. Compared to B-Squad, \system performs better for $9\%$ of relations, and comes within $20$ $F_1$ for another $26\%$ of relations. Compared to B-ZSRE, \system performs better for $6\%$ of relations, and comes within $20$ $F_1$ for another $12\%$ of relations. This shows for certain relations, \system can perform competitively even with supervised models.



% As shown, \system outperforms all unsupervised QA-based methods for all benchmarks yielding performance improvements of up to 27.8 $F_1$ points compared to the next-best method. Moreover, in two out of the four benchmarks (i.e., T-REx and Google-RE) \system yields improvements of 3.3 and 11.4 $F_1$ points compared to the best performing supervised method. {\em These results highlight the fact that structured knowledge can be directly extracted from high-capacity language models without training any fine-tuned extractive models.} However, {\em if we compare the performance of \system with the performance of the Naive Cloze (NC) approach---the gap can be as great as 81.6 $F_1$---we see that we need to associate evidence with the cloze queries to obtain accurate extractions.}

% We discuss performance with respect to different benchmarks. For the single-token benchmarks, Google-RE and T-REx, \it relation mentions, while contexts in T-REx may contain implicit mentions (e.g., a relation like citizenship might only be implied by an adjective describing ethnicity).

% %We see that the performance gap between the best performing of the methods that can reject a context (i.e., \system amongst B-Squad, B-ZSRE, and \system) and the best-performing of the methods that cannot reject context (i.e., UE-QA and SE-QA) increases from 22.9 $F_1$ points to 39.4 $F_1$ points. {\em These results highlight the importance of context rejection: if poor contexts are retrieved and the model extracts a relation forcefully, extractions will be naturally more noisy.} We see that for T-REx, \system outperforms all methods (including the supervised models) yielding more robust extractions.

% For ZSRE and TACRED, we see that while \system outperfosystem outperforms all baselines. {\em These results highlight the efficacy of the token identification component of \system.} {\em The anchor token is consistently the most important token to retrieve.} In contrast to \system, all QA-based methods achieve lower EM and $F_1$ scores. As we demonstrate in Section~\ref{sec:perf_analysis}, the lower accuracy of these methods can be attributed to their tendency to extract longer spans from the given context.

% Comparing the performance of all models for Google-RE to that for T-REx, we find that the EM and $F_1$ scores for all models drop significantly, except for NC. This decrease in accuracy is expected since the contexts in Google-RE contain explicrms the unsupervised methods by more than 20 $F_1$ points, its performance is worse than the supervised BERT methods. We analyze the reason for this gap in the next section where we present an in-depth failure analysis for \system. A promising result, however, is that \system matches the performance of the supervised BiDAF baseline. This result highlights the efficacy of our method.

%\noindent\textbf{Takeaway:} \system can accurately extract structured knowledge directly from a high-capacity language model by evaluating evidence-enhanced cloze queries against the language model.


\subsection{Detailed performance analysis}\label{sec:perf_analysis}
We present an error analysis for \system and competing models. We also provide examples that support these results in Appendix \ref{sec:qual}.


% \begin{figure}
% \center
% \includegraphics[width=0.5\textwidth]{figures/error_qa.pdf}
% \caption{Error categorization of QA-based methods. For \system all errors belong to the No overlap group.}
% \centering
% \label{fig:qa_googlre_trex_error}
% \end{figure}

% \begin{figure}
% \center
% \includegraphics[width=0.5\textwidth]{figures/error_reflex.pdf}
% \caption{Error breakdown of \system.}
% \centering
% \label{fig:zsre_breakdown}
% \end{figure}

\newparagraph{QA Error analysis} We first analyze the errors of the QA-based models in Google-RE and T-REx. We run all models and focus on predictions that do not correspond to exact matches. We further categorize output extractions into groups depending on if there is no overlap with the ground truth span, or by how much longer the prediction span is (recall that for these benchmarks the target span is always a single token). The breakdown of non-exact match predictions in these categories are shown in Figure~\ref{fig:qa_googlre_trex_error} for both benchmarks. Since Google-RE and T-REx focus on single-token extractions, all errors made by \system belong to the No overlap category.

For the supervised QA baselines, we see that most errors in Google-RE correspond to including one or two more tokens in the extracted span (compared to the ground truth span). This indicates that the trained QA heads are biased towards including more information than necessary, which leads to worse performance on the dataset.

In T-REx, we see that a majority of the errors are in the ``No overlap" category. We hypothesize that this is because contexts in T-REx are algorithmically aligned, and may not contain explicit syntactic clues about the answer to the relational query. Without these clues, the performance of the supervised QA heads deteriorate.

We see similar behavior exhibited by the UE-QA baseline, while the SE-QA baseline tends to completely miss the target consistently.

\emph{Our takeaway:} Training on QA pairs adds biases to what information is included in the returned span, as well as a reliance on syntactic clues in order to generalize to unseen examples.

\newparagraph{RE-Flex Error analysis} We focus on ZSRE and TACRED and seek to understand {\em why \system cannot match the performance of the supervised methods B-Squad and B-ZSRE}. We collect all instances for which \system does not predict an exact match with the ground truth. We group errors into four categories: (1) the prediction overlaps with the target span, but is mismatched, (2) the prediction does not overlap with the target span, (3) the model should have rejected the context instead of accepting (should reject), (4) the model should have accepted the context instead of rejecting (should accept). The error breakdown is shown in Figure~\ref{fig:zsre_breakdown}.

We find that most errors can be attributed to \system's context rejection mechanism. We find that the context rejection tends to be more selective about which spans express the relation. We suspect that extending the context rejection to incorporate dependency semantics and word order might lead to a better performance in this area, and leave these explorations as future work,

Comparatively, fewer errors are committed by the anchor token identifier, highlighting the strength of directly using the hidden representations of self-supervised language models.

\emph{Our takeaway:} A majority of error committed by RE-Flex are because of context rejection. Designing more effective measures of whether relations are generally expressed is an important line of future work.

% {\em Automatically-collected training data used by the two unsupervised models introduce significant bias to the span-length of the extractions.} Recall that the QA model in SE-QA is trained to predict entire noun, verb, adjective and named entity phrases, which typically span multiple tokens~\cite{dhingra_simple_2018}. Similarly, the QA model in UE-QA is trained on answer spans that are named entity phrases, which can also contain multiple spans~\cite{lewis_unsupervised_2019}. We suspect that these subtle changes can cause these models to include extraneous information in their extractions.

% We see that the B-ZSRE does not suffer from predicting longer spans. Recall that it is trained over QA pairs created using relations from WikiData, which explains why the bias to the span-length is significantly smaller.

% For T-REx, the error behavior of UE-QA and SE-QA remains the same. However, for B-Squad and B-ZSRE we see that the majority of errors are due to the predicted spans not having any overlap with the correct extraction. We attribute this change in behavior to the fact that contexts in T-REx are not guaranteed to contain an explicit mention of the target relation, which leads to significantly more noisy extractions for B-Squad and B-ZSRE.

% %\begin{figure}[t]
% %\center
% %\includegraphics[width=0.48\textwidth]{figures/cf_qualitative_results.pdf}
% %\caption{Example extractions from ZSRE for the different methods. Here, \textbf{R} indicates the target relation, \textbf{T} the cloze template used, \textbf{Q} the corresponding question required by the QA-based models, and \textbf{C} the provided context for the extraction task.}
% %\centering
% %\label{fig:qual_examples}
% %\end{figure}

% %\noindent\textbf{Takeaway:} The training data used to train the QA model for QA-based relation extraction methods can introduce significant biases to the span-length and quality of the final extractions.

% We focus on ZSRE and TACRED and seek to understand {\em why \system cannot match the performance of the supervised methods B-Squad and B-ZSRE}. We collect all instances for which \system does not predict an exact match with the ground truth. We group errors into four categories: (1) the prediction overlaps with the target span, but is mismatched, (2) the prediction does not overlap with the target span, (3) the model should have rejected the context instead of accepting (should reject), (4) the model should have accepted the context instead of rejecting (should accept)The error breakdown is shown in Figure~\ref{fig:zsre_breakdown}.

% We find that most errors can be attributed to \system's context rejection mechanism. We find that the context rejection tends to be more selective about which spans express the relation. We suspect that extending the context rejection to incorporate dependency semantics and word order might lead to a better performance in this area, and leave these explorations as future work,

% Comparatively, fewer errors are committed by the anchor token identifier, highlighting the strength of directly using the hidden representations of pretrained language models.
%\newparagraph{Qualitative examples}

%Finally, we provide few qualitative examples of extractions from ZSRE obtained by the different methods. The examples are shown in Figure~\ref{fig:qual_examples}. The first two examples highlight two accurate extractions from \system, while the third example an incorrect extraction. These examples also highlight the weakness of the UE-QA and SE-QA methods: many times they extract an incorrect large sequence from the input context.


\begin{table}[t]
\centering
\small
\begin{tabular}{c|c c|c c} 
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{ZSRE}} & \multicolumn{2}{c}{\textbf{TACRED}} \\ \cline{2-5}
& \textbf{EM} & \textbf{$\mathbf{F_1}$} & \textbf{EM} & \textbf{$\mathbf{F_1}$} \\ \hline
No rejection & 40.0 & 43.4 & 39.1 & 39.5 \\ 
With rejection & 43.7 & 46.9 & 49.4 & 50.1 \\ 
\end{tabular}
\caption{Context rejection ablation on ZSRE.}
\label{tab:context_ablation}
\end{table}

\subsection{Micro-benchmarks}\label{sec:micro} 
We evaluate the effect of different components of \system on its end-to-end performance. 
\newparagraph{Context rejection analysis} We first examine the effect of \system's context rejection mechanism on ZSRE. We consider \system's performance with and without context rejection. The results are shown in Table~\ref{tab:context_ablation}. We see that context rejection improves the performance of \system significantly. This result shows that context rejection is necessary for unsupervised relation extraction.

% \begin{figure}[t]
% \center
% \includegraphics[width=0.4\textwidth]{figures/context_filtering_lambda.pdf}
% \caption{\system's overall performance on ZSRE as we varying the context filtering threshold.}
% \centering
% \label{fig:cf}
% \end{figure}

% \begin{figure}[t]
% \center
% \includegraphics[width=0.4\textwidth]{figures/context_filtering_lambda_3rel.pdf}
% \caption{Per-relation breakdown of \system's performance as we vary the context filtering threshold. We show results for three sampled relations from ZSRE.}
% \centering
% \label{fig:3rel}
% \end{figure}

% \begin{figure}
% \center
% \includegraphics[width=0.48\textwidth]{figures/merged_topk_analysis}
% \caption{Effect of parameter $k$ on $F_1$ for Google-RE.}
% %\includegraphics[width=8cm]{Plot}
% \centering
% \label{fig:merged_topk}
% \end{figure}

% Next, we evaluate the the effect of the threshold parameter $\lambda$, which selects the similarity threshold to reject contexts. We first vary $\lambda$ and evaluate \system for all relations in ZSRE. We present the results in Figure~\ref{fig:cf}. We see that the optimal $\lambda$ parameter is 0.0. Finally, we can examine whether the same $\lambda$-value is optimal across relations. 

% We show a per-relation analysis for three sample relations in Figure~\ref{fig:3rel}. We see that the best $\lambda$ varies for each relation, k.

% \begin{table}[t!]
% \centering
% \small
% \begin{tabular}{l|l l|l l}
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{ZSRE}} & \multicolumn{2}{c}{\textbf{TACRED}} \\ \cline{2-5}
% & \textbf{EM} & \textbf{$\mathbf{F_1}$} & \textbf{EM} & \textbf{$\mathbf{F_1}$} \\ \hline
% No expansion  & 42.4 & 46.1 & 49.6 & 50.3 \\ 
% NER expansion  & 36.4 & 39.2 & 42.9 & 43.3 \\ 
% Tuned expansion & 43.7 & 46.9 & 49.4 & 50.1 \\ 
% \end{tabular}
% \caption{Effect of token expansion on ZSRE dataset.}
% \label{tab:tok_expansion}
% \end{table}

\newparagraph{Anchor expansion analysis}
We examine the effect of expanding the anchor token in \system. To examine this behavior in more details, we evaluate \system by considering single-token only extractions, multi-token extractions, and a tuned expansion that chooses either to expand or not to expand based on performance on the development set for each dataset. The results are shown in Table~\ref{tab:tok_expansion}. We see significant deterioration if we consistently expand the anchor token, and very little gain when we turn on expansion on a per relation basis.

%quantify that performance drop by showing both the multi-token and single token performance. Some relations, however, are naturally multi-token, such as the \textit{draftedBy} relation, which expects the location of the sports team as well as the team name. We note for relations like these, the anchor token expansion significantly benefits the extraction. To quantify this benefit, we also present results given an oracle that tells us on a per relation basis whether expanding the anchor token will increase the F1 score of that relation or not. We present the results in Table \ref{table:tokexpansion}.
%
%With the oracle, we see a gain in 3.7 F1 compared to the single token case, showing that selectively using token expansion when needed can be beneficial. As Table \ref{table:1} shows, the expected length of an answer span for this dataset is just under 2 tokens, which implies that the bare minimum answer span should be returned for an exact match. Likely the negative effect of the multi-token expansion is due to the tendency of the expansion models to include too much information across the entire dataset. We verify this claim in Section \ref{section:erroranalysis}.

%\begin{figure}[t]
%\center
%\includegraphics[width=0.48\textwidth]{figures/time_k.pdf}
%\caption{Trade off of approximation parameter k and runtime on the Google-RE dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:k_time}
%\end{figure}

\newparagraph{Approximation analysis}
We examine the tradeoffs between performance, runtime, and the approximation parameter $k$ described in Section~\ref{sec:alignment}. We set the batch size to $1$ to for this analysis. Results are shown in Figure~\ref{fig:merged_topk}. Our measurements show that our choice of $k=16$ leads to high-quality results while it leads to acceptable runtime.

%\subsection{Datasets}
%
%Our 3 datasets are all subsets of Wikidata relations, and are all aligned to contexts in Wikipedia. Thus all pretrained language models used have seen the contexts at pretrain time. The first two datasets are directly pulled from the LAMA probe \cite{petroni_language_2019}, and impose single token constraints on the output. They differ in how the contexts are aligned. Furthermore, neither of these two datasets contain contexts for which the answer does not exist. This gives us a more fair setup to compare against the unsupervised QA models, which cannot predict that an answer is not expressed in the context. The third dataset is designed to be a zero-shot relation extraction benchmark. It contains contexts for which there is no answer to the relational query, and has multi-token spans.
%
%\subsubsection{Google-RE}
%
%Google-RE contains 60k facts manually extracted from Wikipedia. Each fact is aligned to a short context in Wikipedia, then a group of annotators determine if the context expresses the relation, which ensures that the associated context expresses the relation. We define a cloze template and a question for each relation and predict the tail object of the fact. For this dataset we consider the same samples and setup provided in the LAMA probe \cite{petroni_language_2019}. The three relations are \textit{date\_of\_birth}, \textit{place\_of\_birth}, and \textit{place\_of\_death}.
%
%\subsubsection{T-REx}
%
%We consider 41 WikiData relations from the T-REx dataset \cite{elsahar_t-rex:_nodate}, which automatically aligns each fact tuple to a context in Wikipedia. Because the alignment is based on a pipeline, there is no guarantee that the context expresses the relation, unlike Google-RE. We again consider the same samples and relation subset provided by the LAMA probe \cite{petroni_language_2019}. We define a cloze template and a question for each relation and must predict the tail object of the fact.
%
%\subsection{Zero Shot Relation Extraction Benchmark}
%
%The Zero Shot Relation Extraction Benchmark was created by \cite{levy_zero-shot_2017} to test how well relation extraction systems can generalize to unseen relations. The dataset contains 120 WikiData relations, divided by relation into train, validation, and test folds. Relations in the test folds are not present in the train and validation folds. Ten folds are provided, but the test set of the first five folds cover all 120 relations, so we consider the concatenation of the test sets of the first five folds. Each test fold originally contains 12,000 samples and 24 relations, and there is sample overlap between the folds. We filter the concatenated dataset to remove duplicate subject, object, and sentence triplets. We select the first question to appear for each each relation, and define a template for all 120 relations. Final dataset characteristics are provided in table \ref{table:3}. This is the most challenging dataset: systems are expected to reject contexts if they do not express the provided relation, and the expected answer is a variable length span. 
%
%
%\begin{table}[h!]
%\centering
%\begin{tabular}{ |c|c| } 
%\hline
%Total Number of Samples & 42,635 \\
%Number of Relations  & 120 \\
%Number of no answer samples & 17,878 \\
%Number of single token samples & 10,387 \\
%Number of multi token samples & 14,370 \\
%Mean token length & 1.96 \\
%\hline
%\end{tabular}
%\caption{ZSRE Dataset Characteristics}
%\label{table:3}
%\end{table}
%
%\subsection{Baselines}
%
%We now explain our baselines. We primarily compare to extractive QA models, as these do not need to be trained a per relation basis, similar to our model. 
%
%\subsubsection{\cite{lewis_unsupervised_2019}}
%This unsupervised model samples many sentences from a target corpus, masks named entities, then translates the masked clozure statement to a question using an unsupervised Neural Machine Translation model. It then trains a question answering head on top of BERT-large \cite{devlin_bert:_2018}. Similar to our model, it relies on an off the shelf named entity recognition model. However, they use it to collect training data for their question answering head, while we use the NER system optionally to return a multi-token span. It is an unsupervised QA system in the sense that it does not require a user to explicitly provide question-answer training pairs. They provide the training data they use for their system, and we use that to train a BERT-large QA model using the HuggingFace Transformers library [CITE HERE]. Note that this model is designed for the Squad1.0 QA setting, where the question always contains an answer. Therefore, it can never reject a context that does not answer the query.
%
%\subsubsection{\cite{dhingra_simple_2018}}
%
%This model was originally proposed as a semi-supervised approach to question answering. Like \cite{lewis_unsupervised_2019}, they use an off the shelf NER system to generate cloze based question-answer pairs. They train directly on the generated cloze statements (no translation to question), and they only generate examples over introductions of input documents. They also provide their generate training data, which we use to train a BERT-large QA model. Like above, this model is not trained to identify if the query can be answered by a given context.
%
%\subsubsection{BERT-Large trained on Squad2.0}
%
%We train BERT-Large on Squad 2.0 [CITE ME]. Because Squad 2.0 covers a wide array of questions over Wikipedia, there is presumably overlap between the questions asked in our datasets and those asked in the Squad 2.0 dataset. The performance of this model measures how well QA models trained on a QA dataset can generalize to relation extraction queries. As this model is capable of rejecting contexts, for the two datasets where always answering is the optimal behavior we disregard when the model predicts no answer and instead choose the start and end markers with the next highest softmax scores.
%
%\subsubsection{BERT-Large trained on ZSRE benchmark}
%
%We train five BERT-Large models on the first five folds of the ZSRE benchmark. When we measure performance on the ZSRE benchmark, we query each BERT-Large model according to its test relations, as in the zero shot setting. For the other datasets, we simply predict using the first fold's model. For these relations, there is some overlap between a few of the relations as some relations are present in multiple datasets, and thus the model is not truly zero shot. Again, for datasets for which giving an answer is optimal, we disregard when the model predicts no answer. The results of this model measure how well modern QA architectures trained on relation extraction based QA pairs perform in the zero shot setting.
%
%\subsection{Metrics}
%
%Our metrics are the widely adopted exact match (EM) and F1 metrics. Exact match is an aggregate of how many predicted spans are exactly the ground truth, while F1 measures the precision and recall between tokens in the predicted span and tokens in the ground truth span. We average EM and F1 over all samples in each relation to obtain a relation EM and F1, then average over all relation EM and F1 scores to obtain a final dataset EM and F1.
%
%\subsection{Implementation Details}
%
%Unless otherwise stated, we set our $\lambda$ parameter to $1$ and our approximation parameter $k$ to 10. We use the fairseq library's implementation of RoBERTa-large [CITE ME] as our pretrained language model, and use the LAMA probe experiment setup as a starting point for our own experiments. For the embeddings of the context rejection mechanism, we use the FastText library [CITE ME]. For the token embeddings of the alignment model, we first collect an embedding for each subword (RoBERTa uses byte-pair subword encodings) by concatenating the output representation of all 12 of the RoBERTa-large decoder layers for each subword. Because we operate on the token and not the subword level, we obtain a token representation by averaging all subword vector embeddings that compose a token. Examining the effect of our embedding choices is out of the scope of this work, and we leave it as a future direction.
%
%For named entity recognition and noun phrase chunking, we use the default models of the Spacy library [CITE ME].
%
%We train and run all models on a single NVIDIA V100 32GB memory GPU.

%\subsection{Performance on relation extraction}\label{sec:overall}
%
%We present our end to end results on all three datasets in table \ref{table:1}. We can see that RE-Flex outperforms all baselines in the single token setting. This highlights the performance of the anchor identification: the anchor token is consistently the most important token to retrieve. Any extraneous supplementary phrases are augmented at anchor expansion, which in this case is unnecessary. All baselines are penalized for adding additional information in this setting. We further analyze the QA models' tendency to include more information than necessary in section \ref{section:erroranalysis}.
%
%Because the T-REx dataset alignments are done algorithmically, the evidence that the relation is expressed in the supplied context is fundamentally weaker than in the Google-RE dataset, where the supplied context is manually verified to express the relation. As a result, scores for all models significantly drop. This highlights the importance of the context retriever: if poor contexts are retrieved and answers are expected, extractions will be naturally more noisy. Still, RE-Flex outperforms all the other models, and thus is clearly more robust to the quality of retrieved contexts. We believe this is additional evidence of pretrained language models' ability to store relational information. Even if the evidence is weak, the language model is often still able to associate its prediction with the correct part of the context, implying that it is able to implicitly model type information. We further examine the pretrained language model's ability to recognize type in section [FILL ME].
%
%In the ZSRE dataset, we see that RE-Flex significantly outperforms unsupervised QA baselines. Our results in the table are with the multi-token expansion disabled, as enabling it decreases performance. We further analyze this result in sections \ref{section:tokenexpansion} and \ref{section:erroranalysis}. Because the ZSRE dataset has many failure modes for our end to end approach, we further analyze our errors for this dataset in section \ref{section:erroranalysis}.
%
%
%\begin{table}[t]
%\centering
%\begin{tabular}{ |c|c|c|c| } 
%\hline
%Dataset & Model & EM & F1 \\
%\hline
%\multirow{5}{4em}{Google-RE} & RE-Flex & 91.1 & 91.1 \\ 
%& \cite{lewis_unsupervised_2019} & 54.3 & 68.2 \\ 
%& \cite{dhingra_simple_2018} & 25.9 & 34.6 \\ 
%& BERT-Large+Squad2.0 & 53.6 & 77.0 \\ 
%& BERT-Large+ZSRE & 83.2 & 88.2 \\ 
%\hline
%\multirow{5}{4em}{T-REx} & RE-Flex & 67.1 & 67.1 \\ 
%& \cite{lewis_unsupervised_2019} & 13.6 & 18.5 \\ 
%& \cite{dhingra_simple_2018} & 20.8 & 27.7 \\ 
%& BERT-Large+Squad2.0 & 41.2 & 51.0 \\ 
%& BERT-Large+ZSRE & 46.8 & 52.2 \\ 
%\hline
%\multirow{5}{4em}{ZSRE} & RE-Flex & 42.4 & 46.0 \\ 
%& \cite{lewis_unsupervised_2019} & 16.7 & 23.8 \\ 
%& \cite{dhingra_simple_2018} & 17.4 & 25.1 \\ 
%& BERT-Large+Squad2.0 & 66.0 & 73.8 \\ 
%& BERT-Large+ZSRE & 66.5 & 70.2 \\ 
%\hline
%\end{tabular}
%\caption{End to end results}
%\label{table:1}
%\end{table}

%\subsection{Effect of context rejection mechanism}
%
%We examine the effects of the context rejection mechanism on the ZSRE dataset. We first examine performance if we were to remove context rejection entirely in Table \ref{table:2}. We can see that context rejection significantly contributes to performance on the ZSRE dataset, which means that the unsupervised QA baselines without context rejection are currently unsuited for relation extraction. Our performance without the context rejection still outperforms the unsupervised QA baselines, highlighting the strength of our anchor identification model.
%
%We now turn to characterizing the effect of the threshold parameter $\lambda$, which selects the similarity threshold to reject contexts that do not express the input relation. We first vary $\lambda$ for the entire ZSRE dataset, and present the results in Figure \ref{fig:cf}. We see that the optimal $\lambda$ parameter is 0, which implies that half of all given contexts are determined to not express the relation. This roughly aligns with the fact that $41\%$ (see Table \ref{table:1}) of the examples in the dataset have no answer, though clearly the rejection mechanism rejects more than it should optimally.
%
%We can examine whether this dataset wide $\lambda$ is consistent across relations. We show the $\lambda$ values and corresponding relation performance in Table \ref{fig:3rel}. We see that the optimal $lambda$ can change for each relation, showing that the context rejection mechanism's performance varies based on the relation. We leave creating a more adaptive rejection mechanism to future work.
%
%\begin{table}[t]
%\centering
%\begin{tabular}{ |c|c|c| } 
%\hline
%Model & EM & F1 \\
%\hline
%RE-Flex with rejection & 42.4 & 46.0 \\ 
%RE-Flex without rejection & 32.5 & 37.5 \\ 
%\hline
%\end{tabular}
%\caption{Context rejection ablation on ZSRE}
%\label{table:2}
%\end{table}

%\subsection{Effect of anchor token expansion} \label{section:tokenexpansion}
%
%We now examine the effect of expanding the anchor token using an off the shelf NER and noun phrase chunking model. As previously stated, choosing to expand the anchor token decreases the performance of our approach on the ZSRE dataset. We quantify that performance drop by showing both the multi-token and single token performance. Some relations, however, are naturally multi-token, such as the \textit{draftedBy} relation, which expects the location of the sports team as well as the team name. We note for relations like these, the anchor token expansion significantly benefits the extraction. To quantify this benefit, we also present results given an oracle that tells us on a per relation basis whether expanding the anchor token will increase the F1 score of that relation or not. We present the results in Table \ref{table:tokexpansion}.
%
%With the oracle, we see a gain in 3.7 F1 compared to the single token case, showing that selectively using token expansion when needed can be beneficial. As Table \ref{table:1} shows, the expected length of an answer span for this dataset is just under 2 tokens, which implies that the bare minimum answer span should be returned for an exact match. Likely the negative effect of the multi-token expansion is due to the tendency of the expansion models to include too much information across the entire dataset. We verify this claim in Section \ref{section:erroranalysis}.
%
%\begin{table}[t]
%\centering
%\begin{tabular}{ |c|c|c| } 
%\hline
%Model & EM & F1 \\
%\hline
%RE-Flex with multi-token expander & 31.4 & 38.3 \\ 
%RE-Flex with single token & 37.8 & 43.0 \\ 
%RE-Flex with expander Oracle & 41.9 & 46.7 \\ 
%\hline
%\end{tabular}
%\caption{Effect of token expansion on ZSRE dataset}
%\label{table:tokexpansion}
%\end{table}
%
%\subsection{Qualitative examples}
%
%We highlight some qualitative examples in Figure \ref{fig:qualitative}. The first two examples highlight two successes of our approach, while the second highlights a failure. One key aspect of these examples is that they show a key weakness of unsupervised QA baselines: they sometimes highlight a random, large sequence in the input.
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/cf_qualitative_results.pdf}
%\caption{Qualitative results. R is the relation, T is the template required by RE-Flex, Q is the question required by QA baselines. L is the model of \cite{lewis_unsupervised_2019}. D is the model of \cite{dhingra_simple_2018}. BS is BERT-large trained on Squad2.0. BZSRE is BERT-large trained on the ZSRE train set.}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:qualitative}
%\end{figure}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/context_filtering_lambda.pdf}
%\caption{Context filtering graph}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:cf}
%\end{figure}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/context_filtering_lambda_3rel.pdf}
%\caption{$\lambda$ performance tradeoff for three sampled relations from the ZSRE dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:3rel}
%\end{figure}
%
%
%\subsection{Error Analysis} \label{section:erroranalysis}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/googlere_qa_error.pdf}
%\caption{Error categorization of baseline QA Models on the T-REx dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:qa_googlre_error}
%\end{figure}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/trex_qa_error.pdf}
%\caption{Error categorization of baseline QA models on the T-REx dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:qa_trex_error}
%\end{figure}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/ours_error_zsre.pdf}
%\caption{Error categorization of RE-Flex on the ZSRE dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:our_error_zsre}
%\end{figure}
%
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/k_f1.pdf}
%\caption{Trade off of approximation parameter k and F1 on the Google-RE dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:k_f1}
%\end{figure}
%
%\begin{figure}[t]
%\includegraphics[width=0.48\textwidth]{figures/time_k.pdf}
%\caption{Trade off of approximation parameter k and runtime on the Google-RE dataset}
%%\includegraphics[width=8cm]{Plot}
%\centering
%\label{fig:k_time}
%\end{figure}
%
%We now seek to verify previously made claims with respect to the behavior of our model and that of our baselines. We first analyze the errors of the QA models in the Google-RE dataset and and a subset of 10 random relations in the T-REx dataset. We run all models, and collect all results where the exact match of the prediction is not 1. Conditioned on this, we categorize the prediction depending on if there is no overlap with the answer span, or by how much longer the prediction span is (for these datasets, the target span is always of length 1). The breakdown of these errors are shown in Figures \ref{fig:qa_googlre_error} and \ref{fig:qa_trex_error}.
%
%For the Google-RE dataset, we see that for all the models, having no overlap is the most common type of error. The second most common error across all models is returning a span longer than the target span by 5 or more tokens. \cite{dhingra_simple_2018} suffers the most from this type of error, which is likely reflective of the training data they use to train their QA head. They train their QA model to predict entire noun, verb, adjective, and named entity phrases, which can span for many tokens. \cite{lewis_unsupervised_2019}, on the other hand, train on answer spans that are exclusively named entity phrases, which are usually shorter than collective noun, verb, and adjective chunks.
%
%The error distribution significantly changes when considering the T-REx dataset. Here, all models see a drop in the percentage of errors made because of no overlap, and increase the proportion of errors made due to incorrect span length. This is likely the result of changing the quality of the context retrieval. In the presence of weaker evidence, the QA models, with the exception of \cite{dhingra_simple_2018} all return higher length spans. This could be evidence of uncertainty. Another interesting result is that the BERT-large baseline trained on Squad2.0 commits significantly more errors because of returning a span length of length 1 or 2 more than what is required. This shows that this model performs significantly better than the EM and F1 numbers reflect.
%
%We now turn to examine why there is performance deterioration for the RE-Flex model on the ZSRE dataset. We collect all samples for which RE-Flex does not predict an exact match with the ground truth. We enable our multi-token expansion. We categorize our error into five categories: whether the predicted span is of length larger than required, shorter than required, whether the model should have rejected the context when it accepted, whether the model should have accepted the context when it rejected, and whether the predicted anchor token is outside the ground truth span. Results are shown in Figure \ref{fig:our_error_zsre}. The largest portion of error can be attributed to our rejection mechanism: a large portion of the errors committed are because the model rejected when it should have accepted and rejected when it should have accepted. The next most significant error is the anchor being outside the ground truth span, which highlights that our anchor token prediction model is not perfect. Finally, the amount of errors committed because the spans were too long versus too short show that our token expansion still expands tokens too much.

%\subsection{Approximation parameter tradeoffs}
%
%Finally, we examine the tradeoff of performance, runtime, and the approximation parameter $k$ described in section \ref{section:alignment}. Results are show in Figures \ref{fig:k_f1} and \ref{fig:k_time}. Our measurements show that there is not much cost to having the approximation parameter be as low as $10$ on extraction performance, but there is a linear increase in runtime as $k$ increases. This justifies our default value for $k$.
%
%\subsection{Comparison to Snorkel Relation Extraction}
%We contrast RE-Flex with the approach of developing labeling functions and text matchers informed by domain knowledge of the relation to extract the object. Candidate objects were extracted for each relation using regex matching rules. We then wrote labeling functions as part of the Snorkel framework to generate noisy labels for the task of classifying whether or not a sentence expresses the relation. We assume an oracle aware of all information necessary to write effective labeling functions, such as a list of all possible languages for the \textit{native\_language} relation, or a knowledge of common types of vessels for the \textit{vessel\_class} relation. The sentences and generated labels were then used to train an end extraction Bidirectional LSTM model. 
%
%Examples of labeling functions used in the \textit{date\_of\_birth} include using the results of off the shelf NER systems as well as considering features such as proximity to the subject in order to determine the best candidate object in a given sentence. 
%
%\lstset{language=Python}
%\lstset{frame=lines}
%\lstset{caption={NER based labeling function}}
%\lstset{label={lst:code_direct}}
%\lstset{basicstyle=\footnotesize}
%\begin{lstlisting}
%def contains_person(x):
%    doc = nlp(x.sentence)
%    for e in doc.ents:
%        if e.label_ == "PERSON":
%           return POSITIVE
%    return NEGATIVE
%\end{lstlisting}
%\newpage
%\lstset{language=Python}
%\lstset{frame=lines}
%\lstset{caption={Candidate selection}}
%\lstset{label={lst:code_direct}}
%\lstset{basicstyle=\footnotesize}
%\begin{lstlisting}
%def born_close_to_subject(x):
%    sent = x.sentence
%    subj = x.subject
%    if 'born' not in sent: return ABSTAIN
%    if(sent.index('born') - 
%    sent.index(subj) <= 2): 
%        return POSITIVE
%    return NEGATIVE
%\end{lstlisting}
%
%
%We evaluated this technique by determining the existence of a given relation in a sentence using the trained model and comparing the extracted object labels against the ground truth object extractions. The F1 results are described in table \ref{table:5}.
%
%\begin{table}[h!]
%\begin{center}
% \begin{tabular}{|| c c c ||} 
% \hline
% \textbf{Relation} & \textbf{Snorkel} & \textbf{RE-Flex} \\ [0.5ex]
% \hline
% \textit{date\_of\_birth} & .7253 &.4377\\
% \hline
% \textit{vessel\_class} & .8087 & .4083\\
% \hline
% \textit{chromosome} & .9890 & 0.5093\\
% \hline
% \textit{native\_language} & .9060 & 0.6183\\
% \hline
% \textit{position\_played} & .9773 & .7174\\
% \hline
%\end{tabular}
%\caption{Snorkel extraction F1 scores on ZSRE}
%\label{table:5}
%\end{center}
%\end{table}
%
%We observe that creating noisy labels and regex matching results in significantly better F1 performance over our methods across every relation we tried. The differences were especially noticeable in cases such as the \textit{chromosome} relation, which have consistent semantics that are easily matched and only one candidate existed per sentence. However, the effectiveness of this technique is significantly constrained by the need for prior knowledge of the relation domain in order to write effective matchers and labeling functions, unlike RE-Flex. 
%
%
%
%Still in progress
%

